Domain Generalization through the Lens of Angular Invariance

Domain generalization (DG) aims at generalizing a classifier trained on multiple source domains to an unseen target domain with domain shift. A common pervasive theme in existing DG literature is domain-invariant representation learning with various invariance assumptions. However, prior works restrict themselves to a radical assumption for realworld challenges: If a mapping induced by a deep neural network (DNN) could align the source domains well, then such a mapping aligns a target domain as well. In this paper, we simply take DNNs as feature extractors to relax the requirement of distribution alignment. Specifically, we put forward a novel angular invariance and the accompanied norm shift assumption. Based on the proposed term of invariance, we propose a novel deep DG method called Angular Invariance Domain Generalization Network (AIDGN). The optimization objective of AIDGN is developed with a von-Mises Fisher (vMF) mixture model. Extensive experiments on multiple DG benchmark datasets validate the effectiveness of the proposed AIDGN method.

==> Sect/experiment.tex <==
\section{Experiments}

\subsection{Experimental Settings}

\paragraph{Datasets.} To evaluate the effectiveness of the proposed method, we conduct our experiments on four public benchmark datasets. PACS~\cite{li2017pacs} is composed of four domains $d\in \lbrace$photo, art, cartoon, sketch$\rbrace$, containing 9991 images of 7 categories. VLCS~\cite{fang2013vlcs} comprises four photographic domains $d\in \lbrace$VOC2007, LabelMe, Caltech101, SUN09$\rbrace$, with 10729 samples of 5 classes. OfficeHome~\cite{venkateswara2017office} has four domains $d\in \lbrace$art, clipart, product, real$\rbrace$, containing 15500 images with a larger label sets of 65 categories. TerraIncognita~\cite{beery2018terra} comprises photos of wild animals taken by cameras at different locations. Following~\cite{gulrajani2020domainbed}, we use domains of  $d\in \lbrace$L100, L38, L43, L46$\rbrace$, which include 24778 samples and 10 classes.

\paragraph{Evaluation Protocol.} For a fair comparison, we use the training-domain validation set protocol proposed in DomainBed~\cite{gulrajani2020domainbed} for model selection. For training, we randomly split each training domain into 80\% training set and 20\% validation set and choose the model maximizing the accuracy on the overall validation set, then evaluate its performance on the target domain set. The mean and standard deviation of out-of-domain classification accuracy from three different runs with different training-validation splits are reported. 

\paragraph{Implementation Details.} For all datasets, we use ResNet-50~\cite{he2016resnet} pre-trained on ImageNet~\cite{deng2009imagenet} as the feature extractor $\pi$ and one fully connected layer as the classifier $f$.  We construct a mini-batch containing all source domains where each domain has 32 images. We freeze all the batch normalization layers from pre-trained ResNet since different domains in a mini-batch follow different distributions.  The network is trained for 5000 iterations using the Adam~\cite{kingma2015adam} optimizer. To estimate $\delta_{y,\boldsymbol{\phi}}$ and $\mu_{d,y,\boldsymbol{\phi}}$ in AIDGN loss~\eqref{eq:finalOO}, we treat all $\delta_{y,\boldsymbol{\phi}}$ as one single hyperparameter $\delta$, and perform in-batch estimation for the $d$-th domain norm scale parameter, i.e., $\mu_d$, while ignoring the index $y$ and $\boldsymbol{\phi}$. Specifically, we estimate $\mu_d$ by computing the average norm of samples of the $d$-th domain in a minibatch. We do this mainly for two reasons. First, according to the norm shift assumption, domain index $d$ is more relevant to the norm distribution. Secondly, since the feasible label sets and angular sets can be very large,  it is almost impossible to precisely estimate $\mu_{d,y,\boldsymbol{\phi}}$ in a minibatch. Moreover, for the log term in the KL regularizer, we approximate it with a first order Maclaurin's expansion to make the overall objective function convex.  Following~\cite{gulrajani2020domainbed}, we conduct a random search over the joint distribution of AIDGN hyperparameters. More implementation details about data preprocessing techniques, model architectures, hyperparameter search space and experimental environments can be found in the supplementary material.

% \paragraph{Implementation Details.} For all datasets, we use ResNet-50~\cite{he2016resnet} pretrained on ImageNet ~\cite{deng2009imagenet} as backbone and use Adam~\cite{kingma2015adam} optimizer to train the network for 5000 iterations. The initial learning rate is set to 2.5e-5 and the batch size is set to 32. Following~\cite{gulrajani2020domainbed}, we conduct a random search over the joint distributions of PMAG specific hyperparameters. To reduce the search space, we empirically fix $\lbrace u_a, l_a, s, u_m, l_m\rbrace$ as $\lbrace 410, 10, 110, 0.8, 0.4\rbrace$ and do not search for them. Note that the values for $u_a$, $l_a$ and $s$ are obtained by running the ERM algorithm. For PMAG specific hyperparameters, we search $\beta_e \in \left[0.05, 0.5\right]$,  $\beta_s \in \left[0.0, 0.05\right]$, $\lambda_g \in \left[10.0, 25.0\right]$ and $\eta \in \left[1.0, 3.0\right]$.  More implementation details can be found in the supplementary.

\subsection{Benchmark Comparisons}

We compare our proposed AIDGN with 14 available DG methods in  DomainBed~\cite{gulrajani2020domainbed}. Results on PACS, VLCS, OfficeHome and TerraIncognita are reported in Table~\ref{benchmark comparisons}. All the values of baselines are taken from DomainBed when ResNet-50 is used as a backbone network, except that ERM$^\dagger$ is reproduced by us. For all datasets, AIDGN achieves better average out-of-domain accuracy. Particularly, in TerraIncognita, the proposed method achieves 49.4\%, which is significantly better than the most competitive baseline, 48.6\%. Similarly, it is 86.6\% for PACS, 78.9\% for VLCS, and 68.8\% for OfficeHome, all of which outperform the previous best results. Note that our method is compatible with existing ensemble learning methods~\cite{cha2021swad} and we do not compare AIDGN with them for fairness. 

\begin{table*}[ht]
\centering
\scalebox{0.8}{
\begin{tabular}{l|ccccc|ccccc|}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{\textbf{PACS}} & \multicolumn{5}{c|}{\textbf{VLCS}}\\
\cmidrule(l){2-11} & A & C & P & S & Avg & C & L & S & V & Avg \\
\midrule
ERM~\cite{vapnik1999erm} & 84.7 $\pm$ 0.4 & 80.8 $\pm$ 0.6 & 97.2 $\pm$ 0.3 & 79.3 $\pm$ 1.0  & 85.5 & 97.7 $\pm$ 0.4 & 64.3 $\pm$ 0.9 & 73.4 $\pm$ 0.5  & 74.6 $\pm$ 1.3    & 77.5  \\
ERM$^\dagger$~\cite{vapnik1999erm} & 86.5 $\pm$ 0.8 & 79.9 $\pm$ 0.7 & 97.5 $\pm$ 0.1 & 79.3 $\pm$ 1.0  & 85.8 & 98.6 $\pm$ 0.1 & 65.3 $\pm$ 1.4 & 71.2 $\pm$ 1.4  & 76.0 $\pm$ 0.1    & 77.7 \\
IRM~\cite{arjovsky2019irm} & 84.8 $\pm$ 1.3       & 76.4 $\pm$ 1.1       & 96.7 $\pm$ 0.6       & 76.1 $\pm$ 1.0       & 83.5 & 98.6 $\pm$ 0.1       & 64.9 $\pm$ 0.9       & 73.4 $\pm$ 0.6       & 77.3 $\pm$ 0.9       & 78.5                 \\
DRO~\cite{sagawa2019dro} & 83.5 $\pm$ 0.9       & 79.1 $\pm$ 0.6       & 96.7 $\pm$ 0.3       & 78.3 $\pm$ 2.0       & 84.4 & 97.3 $\pm$ 0.3       & 63.4 $\pm$ 0.9       & 69.5 $\pm$ 0.8       & 76.7 $\pm$ 0.7       & 76.7                 \\
Mixup~\cite{wang2020mixup} & 86.1 $\pm$ 0.5       & 78.9 $\pm$ 0.8       & {\bf97.6 $\pm$ 0.1}       & 75.8 $\pm$ 1.8       & 84.6 & 98.3 $\pm$ 0.6       & 64.8 $\pm$ 1.0       & 72.1 $\pm$ 0.5       & 74.3 $\pm$ 0.8       & 77.4                 \\
MLDG~\cite{li2018mldg} & 85.5 $\pm$ 1.4       & 80.1 $\pm$ 1.7       & 97.4 $\pm$ 0.3       & 76.6 $\pm$ 1.1       & 84.9 & 97.4 $\pm$ 0.2       & 65.2 $\pm$ 0.7       & 71.0 $\pm$ 1.4       & 75.3 $\pm$ 1.0       & 77.2                 \\
CORAL~\cite{sun2016coral} & {\bf88.3 $\pm$ 0.2}       & 80.0 $\pm$ 0.5       & 97.5 $\pm$ 0.3       & 78.8 $\pm$ 1.3       & 86.2 & 98.3 $\pm$ 0.1       & 66.1 $\pm$ 1.2       & 73.4 $\pm$ 0.3       & 77.5 $\pm$ 1.2       & 78.8                \\
MMD~\cite{li2018mmd} & 86.1 $\pm$ 1.4       & 79.4 $\pm$ 0.9       & 96.6 $\pm$ 0.2       & 76.5 $\pm$ 0.5       & 84.6 & 97.7 $\pm$ 0.1       & 64.0 $\pm$ 1.1       & 72.8 $\pm$ 0.2       & 75.3 $\pm$ 3.3       & 77.5                 \\
DANN~\cite{ganin2016dann} & 86.4 $\pm$ 0.8       & 77.4 $\pm$ 0.8       & 97.3 $\pm$ 0.4       & 73.5 $\pm$ 2.3       & 83.6 & {\bf99.0 $\pm$ 0.3}       & 65.1 $\pm$ 1.4       & 73.1 $\pm$ 0.3       & 77.2 $\pm$ 0.6       & 78.6             \\
CDANN~\cite{li2018cdann} & 84.6 $\pm$ 1.8       & 75.5 $\pm$ 0.9       & 96.8 $\pm$ 0.3       & 73.5 $\pm$ 0.6       & 82.6 & 97.1 $\pm$ 0.3       & 65.1 $\pm$ 1.2       & 70.7 $\pm$ 0.8       & 77.1 $\pm$ 1.5       & 77.5                 \\
MTL~\cite{blanchard2021MTL} & 87.5 $\pm$ 0.8       & 77.1 $\pm$ 0.5       & 96.4 $\pm$ 0.8       & 77.3 $\pm$ 1.8       & 84.6 & 97.8 $\pm$ 0.4       & 64.3 $\pm$ 0.3       & 71.5 $\pm$ 0.7       & 75.3 $\pm$ 1.7       & 77.2                 \\
SagNet~\cite{nam2021sagnet} & 87.4 $\pm$ 1.0       & 80.7 $\pm$ 0.6       & 97.1 $\pm$ 0.1       & {\bf80.0 $\pm$ 0.4}       & 86.3 & 97.9 $\pm$ 0.4       & 64.5 $\pm$ 0.5       & 71.4 $\pm$ 1.3       & 77.5 $\pm$ 0.5       & 77.8                 \\
ARM~\cite{zhang2020arm} & 86.8 $\pm$ 0.6       & 76.8 $\pm$ 0.5       & 97.4 $\pm$ 0.3       & 79.3 $\pm$ 1.2       & 85.1 & 98.7 $\pm$ 0.2       & 63.6 $\pm$ 0.7       & 71.3 $\pm$ 1.2       & 76.7 $\pm$ 0.6       & 77.6                 \\
VREx~\cite{krueger2021vrex} & 86.0 $\pm$ 1.6       & 79.1 $\pm$ 0.6       & 96.9 $\pm$ 0.5       & 77.7 $\pm$ 1.7       & 84.9 & 98.4 $\pm$ 0.3       & 64.4 $\pm$ 1.4       & {\bf74.1 $\pm$ 0.4}       & 76.2 $\pm$ 1.3       & 78.3                 \\
RSC~\cite{huang2020rsc} & 85.4 $\pm$ 0.8       & 79.7 $\pm$ 1.8       & {\bf97.6 $\pm$ 0.3}       & 78.2 $\pm$ 1.2       & 85.2 & 97.9 $\pm$ 0.1       & 62.5 $\pm$ 0.7       & 72.3 $\pm$ 1.2       & 75.6 $\pm$ 0.8       & 77.1                 \\
\hline
AIDGN (ours) &  87.9 $\pm$ 0.4 & {\bf82.1 $\pm$ 0.2} & {\bf97.6 $\pm$ 0.1} &  78.8 $\pm$ 0.9 & {\bf 86.6} & 98.3 $\pm$ 0.2 & {\bf65.7 $\pm$ 0.4} & 73.1 $\pm$ 0.4 &  {\bf78.7 $\pm$ 0.7} & {\bf 78.9}  \\

\bottomrule
\end{tabular}}
\hspace{1mm}

\scalebox{0.8}{
\begin{tabular}{l|ccccc|ccccc|}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{\textbf{OfficeHome}} & \multicolumn{5}{c|}{\textbf{TerraIncognita}}\\
\cmidrule(l){2-11} & A & C & P & R & Avg & L100 & L38 & L43 & L46 & Avg \\
\midrule
ERM~\cite{vapnik1999erm} & 61.3 $\pm$ 0.7       & 52.4 $\pm$ 0.3       & 75.8 $\pm$ 0.1       & 76.6 $\pm$ 0.3       & 66.5 & 49.8 $\pm$ 4.4       & 42.1 $\pm$ 1.4       & 56.9 $\pm$ 1.8       & 35.7 $\pm$ 3.9       & 46.1                 \\
ERM$^\dagger$~\cite{vapnik1999erm} & 61.2 $\pm$ 0.5       & 52.9 $\pm$ 0.2       & 76.1 $\pm$ 0.4       & 77.5 $\pm$ 0.1       & 66.9 & 48.6 $\pm$ 0.3       & 43.5 $\pm$ 1.4       & 54.2 $\pm$ 1.0       & 36.9 $\pm$ 0.3       & 45.8\\
IRM~\cite{arjovsky2019irm} & 58.9 $\pm$ 2.3       & 52.2 $\pm$ 1.6       & 72.1 $\pm$ 2.9       & 74.0 $\pm$ 2.5       & 64.3 & 54.6 $\pm$ 1.3       & 39.8 $\pm$ 1.9       & 56.2 $\pm$ 1.8       & 39.6 $\pm$ 0.8       & 47.6                 \\
DRO~\cite{sagawa2019dro} & 60.4 $\pm$ 0.7       & 52.7 $\pm$ 1.0       & 75.0 $\pm$ 0.7       & 76.0 $\pm$ 0.7       & 66.0 & 41.2 $\pm$ 0.7       & 38.6 $\pm$ 2.1       & 56.7 $\pm$ 0.9       & 36.4 $\pm$ 2.1       & 43.2                 \\
Mixup~\cite{wang2020mixup} & 62.4 $\pm$ 0.8       & {\bf54.8 $\pm$ 0.6}       & {\bf76.9 $\pm$ 0.3}       & 78.3 $\pm$ 0.2       & 68.1 & {\bf59.6 $\pm$ 2.0}       & 42.2 $\pm$ 1.4       & 55.9 $\pm$ 0.8       & 33.9 $\pm$ 1.4       & 47.9                 \\
MLDG~\cite{li2018mldg} & 61.5 $\pm$ 0.9       & 53.2 $\pm$ 0.6       & 75.0 $\pm$ 1.2       & 77.5 $\pm$ 0.4       & 66.8 & 54.2 $\pm$ 3.0       & 44.3 $\pm$ 1.1       & 55.6 $\pm$ 0.3       & 36.9 $\pm$ 2.2       & 47.7                 \\
CORAL~\cite{sun2016coral} & {\bf65.3 $\pm$ 0.4}       & 54.4 $\pm$ 0.5       & 76.5 $\pm$ 0.1       & 78.4 $\pm$ 0.5       & 68.7 & 51.6 $\pm$ 2.4       & 42.2 $\pm$ 1.0       & 57.0 $\pm$ 1.0       & 39.8 $\pm$ 2.9       & 47.6                 \\
MMD~\cite{li2018mmd} & 60.4 $\pm$ 0.2       & 53.3 $\pm$ 0.3       & 74.3 $\pm$ 0.1       & 77.4 $\pm$ 0.6       & 66.3 & 41.9 $\pm$ 3.0       & 34.8 $\pm$ 1.0       & 57.0 $\pm$ 1.9       & 35.2 $\pm$ 1.8       & 42.2                 \\
DANN~\cite{ganin2016dann} & 59.9 $\pm$ 1.3       & 53.0 $\pm$ 0.3       & 73.6 $\pm$ 0.7       & 76.9 $\pm$ 0.5       & 65.9 & 51.1 $\pm$ 3.5       & 40.6 $\pm$ 0.6       & 57.4 $\pm$ 0.5       & 37.7 $\pm$ 1.8       & 46.7                 \\
CDANN~\cite{li2018cdann} & 61.5 $\pm$ 1.4       & 50.4 $\pm$ 2.4       & 74.4 $\pm$ 0.9       & 76.6 $\pm$ 0.8       & 65.8 & 47.0 $\pm$ 1.9       & 41.3 $\pm$ 4.8       & 54.9 $\pm$ 1.7       & 39.8 $\pm$ 2.3       & 45.8                 \\
MTL~\cite{blanchard2021MTL} & 61.5 $\pm$ 0.7       & 52.4 $\pm$ 0.6       & 74.9 $\pm$ 0.4       & 76.8 $\pm$ 0.4       & 66.4 & 49.3 $\pm$ 1.2       & 39.6 $\pm$ 6.3       & 55.6 $\pm$ 1.1       & 37.8 $\pm$ 0.8       & 45.6                 \\
SagNet~\cite{nam2021sagnet} & 63.4 $\pm$ 0.2       & {\bf54.8 $\pm$ 0.4}       & 75.8 $\pm$ 0.4       & 78.3 $\pm$ 0.3       & 68.1 & 53.0 $\pm$ 2.9       & 43.0 $\pm$ 2.5       & {\bf57.9 $\pm$ 0.6}       & 40.4 $\pm$ 1.3       & 48.6                 \\
ARM~\cite{zhang2020arm} & 58.9 $\pm$ 0.8       & 51.0 $\pm$ 0.5       & 74.1 $\pm$ 0.1       & 75.2 $\pm$ 0.3       & 64.8 & 49.3 $\pm$ 0.7       & 38.3 $\pm$ 2.4       & 55.8 $\pm$ 0.8       & 38.7 $\pm$ 1.3       & 45.5                 \\
VREx~\cite{krueger2021vrex} & 60.7 $\pm$ 0.9       & 53.0 $\pm$ 0.9       & 75.3 $\pm$ 0.1       & 76.6 $\pm$ 0.5       & 66.4 & 48.2 $\pm$ 4.3       & 41.7 $\pm$ 1.3       & 56.8 $\pm$ 0.8       & 38.7 $\pm$ 3.1       & 46.4                 \\
RSC~\cite{huang2020rsc} & 60.7 $\pm$ 1.4       & 51.4 $\pm$ 0.3       & 74.8 $\pm$ 1.1       & 75.1 $\pm$ 1.3       & 65.5 & 50.2 $\pm$ 2.2       & 39.2 $\pm$ 1.4       & 56.3 $\pm$ 1.4       & {\bf40.8 $\pm$ 0.6}       & 46.6                 \\
\hline
AIDGN (ours) & 64.9 $\pm$ 0.3 & 54.7 $\pm$ 0.3 & 76.5 $\pm$ 0.2 & {\bf79.1 $\pm$ 0.2} & {\bf68.8} & 54.7 $\pm$ 1.8 & {\bf46.8 $\pm$ 1.1} & 57.6 $\pm$ 0.8 & 38.5 $\pm$ 0.8 & {\bf49.4}  \\

\bottomrule
\end{tabular}}
\caption{\textbf{Benchmark Comparisons.} Out-of-domain classification accuracies(\%) on PACS, VLCS, OfficeHome and TerraIncognita are shown. Note that the reuslts of ERM$^\dagger$ are reproduced by us, and other numbers are from DomainBed ~\cite{gulrajani2020domainbed}.}
\label{benchmark comparisons}
\end{table*}

\subsection{Ablation Studies}

To verify the effectiveness of all components of the AIDGN optimization objective, we do ablation studies on the VLCS dataset. Specifically, we compare AIDGN with three variants: a)AIDGN w/o R: The model is trained without the KL regularizer.  b)AIDGN w/o D: The model is trained without estimation for the source domain norm scale parameters, i.e., ignoring the $\mu_d$ term in the expression of $w(r|\boldsymbol{\phi},d,y)$. c)AIDGN w/o RD: The model is trained without both. The results are reported in~\ref{ablation studies}. Note that the results for all the three variants also follow the training-domain validation set model selection and hyperparameter random search protocol, and are obtained from three different runs with different dataset splits. From the results, we can find the full model AIDGN outperforms all these variants, indicating that both the KL regularizer and the estimation for the source domain norm scale parameters are essential to our algorithm.  

\begin{table}[ht]
\centering
\scalebox{0.74}{
\begin{tabular}{lccccc}
\toprule
  & C & L & V & S & Avg \\
\midrule
AIDGN w/o RD & 96.9 $\pm$ 0.3 & 63.5 $\pm$ 0.5 & 73.0 $\pm$ 0.5 & 75.8 $\pm$ 0.6 & 77.3 \\
AIDGN w/o R & 97.3 $\pm$ 0.5 & 64.9 $\pm$ 0.8 & {\bf73.4 $\pm$ 0.4} & 77.9 $\pm$ 1.0 & 78.4  \\
AIDGN w/o D & 97.6 $\pm$ 0.3 & 64.7 $\pm$ 0.4 & {\bf73.4 $\pm$ 0.4} & 78.1 $\pm$ 0.7 & 78.3  \\
AIDGN   & {\bf98.3 $\pm$ 0.2} & {\bf65.7 $\pm$ 0.4} & 73.1 $\pm$ 0.4 & {\bf78.7 $\pm$ 0.7} & {\bf78.9}  \\

\bottomrule
\end{tabular}}
\caption{\textbf{Ablation studies.} Out-of-domain classification accuracies(\%) with different optimization components on VLCS are shown.}
\label{ablation studies}
\end{table}



\subsection{Qualitative Results}


==> Sect/intro.tex <==
\section{Introduction}
Over the past few years, supervised deep learning (DL) has achieved remarkable success on challenging visual tasks~\cite{long2015fully,he2016resnet}%~\cite{krizhevsky2012imagenet,long2015fully,he2016resnet}
. An underlying assumption of the popular supervised DL methods is the identically distributed condition. Namely, the generating functions of training data and testing data are identical. We say there exists a \textit{dataset shift} between the training data (\textit{source domain}) and the testing data (\textit{target domain}) if the identical condition is violated. When there is a dataset shift, the favored empirical risk minimization (ERM) learning \cite{vapnik1999erm} would be ill-posed, since the empirical risk over the training data is not guaranteed to converge to the risk of the testing data asymptotically.

Domain generalization (DG) is a class of inductive learning methods that aims at  learning a classifier minimizing the target risk on the presence of dataset shift \cite{quinonero2009dataset,blanchard2011generalizing}. The inductive setting of DG assumes no target data is available during training, differentiating DG from the transductive domain adaptation methods \cite{ben2007analysis,ganin2015unsupervised}, and thus making DG more practical and challenging. 

Intuitively, in order to carry out a successful knowledge transfer from some "seen" source domains to an "unseen" target domain, there has to be some underlying similarities between these domains. From a theoretical standpoint, invariance between generating functions of domains should be investigated. To this end, a predominant stream in DG is domain-invariant representation learning, with various assumptions on dataset shift such as \textit{covariate shift} assumption~\cite{li2018mmd}, \textit{conditional shift} assumption~\cite{li2018cdann} and \textit{label shift} assumption~\cite{liu2021ijcai21}. 

Formally, denote the original input-output space by $\mathcal{X}\times \mathcal{Y}$. A domain can be identified by the probabilistic measure $\mathcal{P_{X\times Y}}$. Let $\{\mathcal{P_{X\times Y}}^{S_j}\}_{j=1}^N$ denote a set of source domains and $\mathcal{P_{X\times Y}}^T$ denote a target domain respectively. Existing domain-invariant representation learning methods aim to learn a feature mapping $\pi: \mathcal{X} \rightarrow \mathcal{Z}$ from the original input space $\mathcal{X}$ to a latent representation space $\mathcal{Z}$, such that the push forward measures $\{\pi_{*} \mathcal{P_{X\times Y}}^{S_j}\}_{j=1}^N\cup\{\pi_{*} \mathcal{P_{X\times Y}}^T\}$ induced by $\pi$ are identical. For example, the covariate shift assumption manifests itself as $\mathcal{P_{X}}^{S_j}\neq \mathcal{P_{X}}^T$, while invariance holds for the conditional measures $\mathcal{P_{X|Y}}^T=\mathcal{P_{X|Y}}^{S_j},j=1,\ldots,N$. If there exists a feature map $\pi$ satisfying identical push forward marginal measures $\pi_{*} \mathcal{P_X}^{S_j}=\pi_{*} \mathcal{P_X}^T$, then such a $\pi$ satisfies identical push forward joint measures $\pi_{*} \mathcal{P_{X\times Y}}^{S_j}=\pi_{*} \mathcal{P_{X \times Y}}^T$. 

However, those domain-invariant representation learning methods restrict themselves on making invariance assumptions on the original input-output space, and thus resulting in an impractical  
pursuing on identical push forward joint measures for real-world challenges, as ~\cite{gulrajani2020domainbed} showed that few DG algorithms outperform ERM significantly under a fair evaluation protocol.

In this paper, we take a step back from pursuing identical push forward measures, by estimating the relative difference between target distribution and source distributions in the latent space under mild assumptions instead. Specifically, based on a novel angular invariance assumption, we propose a novel paradigm of dataset shift: the \textbf{norm shift}. The norm shift assumption says that the relative difference between the push forward measures induced by a deep neural network feature map is captured by the norm parameters under a polar reparametrization. The norm shift assumption is inspired by the recent finding that the internal layers in a deep neural networks capture high level semantic concepts (e.g. eye, tail) \cite{zeiler2014visualizing,gonzalez2018semantic}. The forward pass of an input in a trained DNN can be viewed as a process of concepts matching, and a higher magnitude of an activation indicates a higher level of concept matching for that particular neuron. Moreover, high level semantic concepts are often related to categorical discriminative concepts. Thus one could expect significant activations when applying the feature map to the target domain, and indeed this expectation is verified by the impressive results achieved by ERM ~\cite{gulrajani2020domainbed}. In DG, the feature map is trained on the source domains, therefore the semantic concepts memorized by the internal layers is biased to the source domains, thus we expect a different magnitude of norms of latent representations between a source domain and a target domain. In Fig. %这段要再表述融合图示和visualization  
% \begin{figure*}[htbp]
%     \centering
%     \subfigure[ERM(domain)]{
%     \begin{minipage}{5cm}
%     \centering
%         \includegraphics[width=5cm]{figure/ERM-domain1.png}
%     \end{minipage}
%     }
%     \subfigure[ERM(class)]{
%     \begin{minipage}{5cm}
%     \centering
%         \includegraphics[width=5cm]{figure/ERM-class1.png}
%     \end{minipage}
%     }
%     \subfigure[norm shift]{
%     \begin{minipage}{5.9cm}
%     \centering
%         \includegraphics[width=5.9cm]{figure/norm-shift.PNG}
%     \end{minipage}
%     }
% \caption{}
% \label{fig1}
% \end{figure*}

Apart from the novel angular invariance and norm shift assumption, our methodological contribution is manifested by a novel deep DG learning algorithm \textbf{A}ngular \textbf{I}nvariance \textbf{D}omain \textbf{G}eneralizaiton \textbf{N}etwork (AIDGN). Aiming at a practical deployment of the proposed angular invariance within a DNN architecture, the designing principle of the AIDGN framework is a minimal level of modification of ERM learning under a modest intensity of distribution assumptions. Concretely,
\begin{enumerate}
    \item We derive an analytic form of $\frac{p^T(Z=z)}{p^{S}(Z=z)}$, which is the ratio between the target and source probability density functions (p.d.f.) in the latent representation space.
    \item Within a von-Mises Fisher (vMF) mixture model \cite{gopal2014mises,taghia2014bayesian}, we derive an AIDGN optimization objective that emphasizes a $\frac{p^T(Z=z)}{p^{S}(Z=z)}$ re-weighted probability of correct prediction. In particular, the proposed optimization objective follows a maximum entropy principle for the label distribution. %Therefore the AIDGN framework differs from the deep DG methods that is based on the balance weight assumption
    \item We demonstrate theorectically that the proposed AIDGN is a generalized form of the recent proposed MAG loss \cite{meng2021magface}. We also give a relative entropy interpretation of the heuristic hyperbolic regularizer.
    \item We conduct extensive experiments to validate the effectiveness of the proposed AIDGN framework on multiple DG benchmarks, and demonstrate its superior performance over the existing DG baselines.
\end{enumerate}


\iffalse
Our main contributions are summarized as follows: 
\begin{itemize}
\item We propose a novel and moderate norm shift assumption compatible with DL. Based on the assumption, we design an effective method which learns the target risk minimizer under the framework of dynamic importance weighting.
\item
\item We theoretically justify the generalized MagFace???
\item We empirically validate the effectiveness of the proposed method on multiple DG benchmarks and demonstrates its superior performance over the comparison baselines.
\end{itemize}


identical push forward joint measure pursuing and invariance assumed on the original input-output space are too restrictive for real-world challenges, as ~\cite{gulrajani2020domainbed} showed that few DG algorithms outperform ERM significantly under a fair evaluation protocol.

these assumptions maybe too restrictive or loose for real-world challenges and lack a precise depiction of inter-domain invariance, as ~\cite{gulrajani2020domainbed} showed that few DG algorithms outperform ERM significantly under a fair evaluation protocol.

Denote by $\mathcal{P^T}$ and $\mathcal{P}^S$ the target domain and a source domain respectively. Let $\pi: \mathcal{X} \rightarrow \mathcal{Z}$ be a feature map from the original input space to a latent representation space. The domain-invariant representation learning methods makes various assumptions on the probability measures $\{\mathcal{P^T}\}\cup\{\mathcal{P}^S_j|j=1,\ldots,N\}$, 


on the push forward measures $\{\pi_{*} \mathcal{P}^T(Z,Y)\}\cup\{\pi_{*} \mathcal{P}^S_j(Z,Y)|j=1,\ldots,N\}$ induced by $\pi$ and $\{\mathcal{P^T}\}\cup\{\mathcal{P}^S_j(Z,Y)|j=1,\ldots,N\}$, where $\mathcal{P^T}$ and $\mathcal{P}^S_j(Z,Y)$ denote the target domain and the $j$-th source domain respectively. For example, the \textit{covariate shift} assumption assumes that the marginals in the $\pi_{*}$ 

with various assumptions on domain shift such as covariate shift assumption~\cite{li2018mmd}, concept shift assumption~\cite{li2018cdann} and conditional shift assumption~\cite{liu2021ijcai21}. However, these assumptions maybe too restrictive or loose for real-world challenges and lack a precise depiction of inter-domain invariance, as ~\cite{gulrajani2020domainbed} showed that few DG algorithms outperform ERM significantly under a fair evaluation protocol.

The domain-invariant representation learning methods focus on the joint distribution of the category variable and the latent representation output by the last convolution layer. 

Suppose that $\mathcal{D}_s=\lbrace\mathcal{D}_1, ..., \mathcal{D}_N\rbrace$


The domain-invariant representation learning methods focus on the joint distribution of the category variable and the latent representation output by the last convolution layer. which are shown to capture high level of semantic concepts (e.g. eye, tail) \cite{zeiler2014visualizing,gonzalez2018semantic}

regard convolutional layers as feature extractors and latent representations are shown to capture high level of semantic concepts (e.g. eye, tail) \cite{zeiler2014visualizing,gonzalez2018semantic}. and focus on the joint distribution of the output latent representations,  

Then, different invariance and shift assumptions on the joint distribution of the latent representation and category variable





Adopting the convolutional layers as feature

Fortunately, studies have shown that the outputs of internal layers in deep neural network capture semantic, and deeper layers 

By leveraging the powerful feature extraction capability of deep neural networks

From a theoretical standard point, 
a predominant stream in DG is domain-invariant representation learning \cite{li2018mmd,li2018cdann,liu2021ijcai21}, which leverages the powerful feature extraction capability of deep learning



 formal assumptions on dataset shift and invariance of
%A predominant stream in DG is domain-invariant representation learning, with various assumptions on domain shift such as covariate shift assumption~\cite{li2018mmd}, concept shift assumption~\cite{li2018cdann} and conditional shift assumption~\cite{liu2021ijcai21}. However, these assumptions maybe too restrictive or loose for real-world challenges and lack a precise depiction of inter-domain invariance, as ~\cite{gulrajani2020domainbed} showed that few DG algorithms outperform ERM significantly under a fair evaluation protocol.

[Ref from chealsea finn that stenghtens the importance of invariance] 




% 随着深度学习【ref hinton06】的发展，有监督学习在图像识别等任务上取得了非凡进步【ref 如alexnet resnet】。但有实践[ref]和理论[ref]上的研究指出,当存在dataset shift时，即当target domain for testing 和 source domain for training 违反有监督学习常用的同分布假设时，通过源域训练得到的classifier在目标域上的generalization performance 会不理想[ref]。Domain adaptation【ref】和domain generalization [ref]是两种处理dataset shift 的学习范式，两者区别是DA是transductive learning而DG是inductive learning，即DG不需要在测试前 know instance covariates in adavance，这使得DG在online学习等场景下具有更好的普适性。 

%Concretely speaking，（半形式化地给出DG的problem formulation）。

%There is a long line of DG literatures over the last decade, 如 domain-invariant feature learning[ref abcd], 如 domain disentanglement feature learning [ref abcd], 如 data augmentation methods [ref abcd]等等。这些方法都或显式或隐式地假设target domain 落在 source domains span 出来的convex hull中。而在真实环境中，target domain 可能不是source domains的内插（interpolation）而是source domains 的外插（extrapolation），这使得上述方法本质上与marginalize 域随机变量的naive的erm 优化类似，且有实践表明[ref domainbed]，在更严苛的测试protocol 下，上述这些方法的performance与erm 没有significance区别。

%（为了弱化target domain extrapolation问题），近期，有一类新方法做test-time adaptation[ref abc]:在测试阶段，基于entropy minimization对在源域训练得到的classifier进行微调。如iclr tent 通过微调BN参数、nips21 ref T3A 通过构造pseudo prototype adjusts the weight of the linear classifier in DNN，以实现 decision boundaries 远离 high-data density region。

% 然而，基于entropy minimization 的test-time adaptation 方法  ！！！！！core insight！！！！

% insight 图 insight 说明

% domain quality measure + instance quality measure

% method 简述

% contribution 总结




%% 切入点：entropy minimization; data uncertainty; decision boundary; smoothness; robustness

%% 逻辑：[earlier literature< ERM]   <--    [test-time adaptation adjusts ERM classifier by entropy minimization]     <--   [entropy minimization and predictive uncertainty minimization]  <--？ [problem! predictive uncertainty decomposes into model uncertainty and data uncertainty (不可消除不确定性)， minimizing data uncertainty introduce undesirable bias ]  && [ on the other hand, by introducing the modeling of data uncertainty -> introduce desirable properties : A) B) C) ...]      
% ====> [necessity of modeling data uncertainty in the training phase] <--- [how to model uncertainty?]  [not trial] [why in our form?]

%% key points: over-confident classifier and biased pseudo-labeling function, absence of uncertainty modeling, data uncertainty and observational noise, modeling observational noise in multiple scopes/granularities（英文用法准确？？）: A) example-wise scope; B) domain-wise scope 

%%% re-formalizing our optimization objective as an importance weighting method, where the norm of an instance carries information about its importance
%%% KEY CONTRIBUTION: a novel term of invariance (There has to be some underlying term of invariance, otherwise distributional shift is impossible to deal with)

For a fixed, deterministic and invertible transformation $\pi: \mathcal{X} \times \mathcal{Y} \rightarrow \mathcal{Z}, x \times y \mapsto z $, let $p_{te}(Z)$ and $p_{tr}(Z|D)$ be the $\pi$-pushed forward (conditional) probability density functions of $p_{te}(X,Y)$ and $p_{tr}(X,Y|D)$ respectively.

Suppose that $supp(p_{te}) \subset supp(p_{tr}(\cdot|d^j))$ for $j=1,\ldots,J$. Let 
\begin{equation}
    w(Z|D=d^j)\triangleq \frac{p_{te}(Z)}{p_{tr}(Z|D=d^j)}.
\end{equation} 
According to Theorem 1 in \cite{fang2020rethinking},
\begin{equation}
    w(Z|D)=\frac{p_{te}(X,Y)}{p_{tr}(X,Y|D)}.
\end{equation}
Invoking $1=\sum_{j=1}^J p_{tr}(D=d^j)$ (Introducing an extra dummy variable denoting training/testing split would be neater and less misleading), it is straightforward to verify
\begin{equation}
    p_{te}(Z)=\sum_{j=1}^J p_{tr}(Z,D=d^j) w(Z|D=d^j)
\end{equation}

%!!!!!!Remark: the key insight here is that $w(Z|D=d^j)$ is not necessarily equals to $1$ as in dataset un-shifted situation, $p_{te}(Z)=p_{tr}(Z)=\sum_{j=1}^J P(Z,D=d^j)$. In other words, when $p_{te}(Z)\neq p_{tr}(Z)$, $Z$ matters!

Then minimizing the target risk $R_{te}(f_{\theta})$ of a classifier $f_{\theta}$,
\begin{equation}
R_{te}(f_{\theta}) =  \mathbb{E}_{p_{te}} \left[\ell(f_{\theta},Z)\right],
\end{equation}
is equivalent to minimizing the importance weighted source risk 
\begin{equation}
\tilde{R}_{tr}(f_{\theta}) \triangleq  \mathbb{E}_{Z \times D} \left[w(Z|D)\ell(f_{\theta},Z)\right].
\end{equation}
Given a sample from source distribution, we may optimize the empirical estimation
\begin{equation}
\widehat{\tilde{R}_{tr}(f_{\theta})}=\sum_{i=1}^n w(z_i|d_i)\ell(f_\theta,z_i)  \approx  \mathbb{E}_{Z\times D} \left[w(Z|D)\ell(f_{\theta},Z)\right] 
\end{equation}

Unfortunately, we have no access to the target distribution in the setting of domain generalization. There is no way to estimate $w(Z|D)$ directly and proper prior assumption is necessary.  

%%%%%%%% the above analysis is solid%%%%%%%%  the below analysis is not solid %%%%%%%%%%

A mild assumption is $p_{te}(Z)\neq p_{tr}(Z|D=d^j)$ for $j=1,\ldots,J$ and $p_{te}(Z)=p_{tr}(Z)=\sum_{j=1}^J p_{tr}(Z,d^j)$, we name the aforementioned assumption the \textbf{globally unshifted} assumption.

Now, we need to justify the following (really challenging in term of rigorous analysis, took me a day or two but nothing persuasive come out)
\begin{equation}
   \begin{aligned}
&w(z_i|d_i)=\frac{p_{tr}(z_i)}{p_{tr}(z_i|d_i)}%=\frac{\sum_{j=1}^J p_{tr}(z_i|d^j)p(d^j)}{p_{tr}(z_i|d_i)}
=p_{tr}(d_i)+\frac{\sum_{j\neq i}^J p_{tr}(z_i|d^j)p_{tr}(d^j)}{p_{tr}(z_i|d_i)}\\
&\propto m(z_i,d_i)=\frac{u_m-l_m}{u_a-l_a}(\|z_i\|_2+\beta_e d_{mean}-\beta_s d_{std})+l_m    
\end{aligned} 
\end{equation}

(or we consider $w(z_i|d_i)\ell(f_{\theta},z_i)$ as a whole)

Notice that an underlying assumption is that $p_{tr}(z_i,d_i)=1/n_{tr}$, then
\begin{equation}
    w(z_i|d_i)%=\frac{p_{tr}(z_i)}{p_{tr}(z_i|d_i)}
    =\frac{p_{tr}(z_i)p_{tr}(d_i)}{p_{tr}(z_i,d_i)}=n_{tr}p_{tr}(z_i)p_{tr}(d_i)
\end{equation}
Intuitively, $p_{tr}(z_i) \propto \|z_i\|_2$, $p(d_i)$ is estimable from the training set. Following this path, it is really weird that the importance weighting term turn out to be like Eq. (7) . So we should not use $p_{tr}(z_i,d_i)=1/n_{tr}$ here. Anyway, it is quite a rough empirical estimation.

% Maybe the globally unshifted assumption should be revised! (Shit............) or some further assumption is needed (Shit again..........)

An information theoretic point of view, 
\begin{equation}
\log w(z_i|d_i)=\log (p_{tr}(z_i))-\log (p_{tr}(z_i|d_i)),
\end{equation}
%$\log w(z_i|d_i)$ encodes extra bits for not knowing domain informaiton $d_i$.
%Then $KL(p_{tr}(Z)\| p_{tr}(Z|d^j))=\mathbb{E}_{p_{tr}(Z)} \log w(Z|d^j)$ is the expected extra bits of not witnessing the $j$-th domain $D=d^j$.%(说反了)
According to the minimum description length (MDL) principle, $KL(p_{tr}(Z)\| p_{tr}(Z|d^j))$ shoud be as small as possible. And by varying $j=1,\ldots,J$, $\sum_{j=1}^J KL(p_{tr}(Z)\| p_{tr}(Z|d^j))$ shoud be as small as possible. 

The MDL solution is achieved when all source domains are from the same data generating distribution, which violates the fundamental assumption of DG.

%%%%%%%%%%%%%%%%%%%
The introduction of the norm function of $Z$ requires a polar transformation for a rigorous derivation (Not trivial, invoking n-sphere jacobian formula and mathematical induction).
\fi

==> Sect/method.tex <==
\section{Methodology}
In this section, we first formulate the DG problem. Secondly, we explain the proposed angular invariance and norm shift assumption. Lastly, we introduce our angular invariance domain generalization network (AIDGN). %Lastly, we conclude this section with an analysis of the loss of AIDGN. 
(\textit{Proofs for this section can be found in the supplementary material.})

%\noindent\textbf{Problem Formulation}\\
\subsection{Problem Formulation}
Give $N$ different source domains $\{\mathcal{P}_{\mathcal{X \times Y}}^{d}\}_{d=1}^N$ and a target domain $\mathcal{P}_{\mathcal{X \times Y}}^{t}$ on the input-output space $\mathcal{X\times Y}$. DG tasks assume $\mathcal{P}_{\mathcal{X \times Y}}^{d}\neq \mathcal{P}_{\mathcal{X \times Y}}^{t}$ for $d=1,\ldots,N$ and focus on $C$-class single label classification tasks. %The output space $\mathcal{Y}$ is often taken as the space of one-hot vectors. 
Let $\mathcal{H}=\{h_{\theta}|\theta \in \Theta\}$ be a hypothesis space parametrized by $\theta \in \Theta$. 
For $d=1,\ldots,N$, there are $n_d$ independently identically distributed instances $\lbrace (\textbf{x}_i^d, y_i^d)\rbrace_{i=1}^{n_d}$ sampled from the $d$-th source domain $\mathcal{P}_{\mathcal{X \times Y}}^{d}$.
The goal of DG is to output a classifier $\hat{h}\in\mathcal{H}$ such that the target risk is minimized for a given loss $\ell\left(h(\cdot),\cdot\right)$, i.e.,
\begin{equation}\label{eq:goal}
    \hat{h}=\arg \min_{h\in\mathcal{H}} \mathbb{E}_{\mathcal{P}_{\mathcal{X \times Y}}^{t}}\left[\ell(h(\textbf{X}),Y)\right].
\end{equation}
%In domain generalization (DG), we have a training set of $N$ source domains $\mathcal{D}_s=\lbrace\mathcal{D}_1, ..., \mathcal{D}_N\rbrace$ with $n_d$ labelled samples $\lbrace (x_i^d, y_i^d)\rbrace_{i=1}^{n_d}$ in the $d$-th domain, where $x_i^d$ denotes the input sample and $y_i^d\in\lbrace1, ..., K\rbrace$ denotes the classification label. The goal of DG is to learn a model on $\mathcal{D}_s$ that can perform well on an unseen target domain $\mathcal{D}_t$.

%\noindent \textbf{The Angular Invariance and Norm Shift Assumption}\\
\subsection{Angular Invariance and Norm Shift}
Celebrated for capturing empirical universal visual features, convolutional neural networks (CNNs) pretrained on the ImageNet dataset~\cite{deng2009imagenet} have been adopted by a wide range of visual tasks [References]. To take full advantage of a pretrained CNN $\pi$, we regard $\pi$ as a feature extractor from the original input space $\mathcal{X}$ to a latent representation space $\mathcal{Z}$. Then a hypothesis $h$  composes of a feature extractor $\pi$ and a classifier $f$, i.e., $h=f\circ\pi$.

Studies have shown that each dimension of a CNN $\pi$ output is capturing some abstract concept (e.g. eye, tail)~\cite{zeiler2014visualizing,gonzalez2018semantic}. Considering the relationship among concepts of the same class objects in the real-world is stable, the angular invariance and norm shift assumption says that the $\pi$-mapped feature of different domains are invariant in the angular parameters, but varies in the norm parameter. For ease of illustration, we introduce a random variable $D$ indexing the $d$-th source domain if $D=d$. Formally, the proposed assumption states as follows.

\begin{assumption}[angular invariance]\label{assump:angularInvariance}
Suppose the marginal distributions $\{\mathcal{P}_{\mathcal{X}}^{d}\}_{d=1}^N\cup\{\mathcal{P}_{\mathcal{X}}^t\}$ on the input space $\mathcal{X}$ are continuous. Let $\pi:\mathcal{X}\rightarrow \mathcal{Z}\subset \mathbb{R}^n$ be a feature extraction map such that the $\pi$-push forward probability density funcitons (p.d.f.s) $\{p^{d}(\textbf{z})\}_{d=1}^N\cup\{p^t(\textbf{z})\}$ exist in the latent space $\mathcal{Z}$. Let $(r,\phi_1,\ldots,\phi_{n-1})=g(z_1,\ldots,z_n)$ be the polar reparametrization \cite{blumenson1960derivation} of the Cartesian coordinates $\textbf{z}=(z_1,\ldots,z_n)$. The angular invariance assumption for DG is quantified by the equations: Let $\boldsymbol{\phi}=(\phi_1,\ldots,\phi_{n-1})$, for $d=1,\ldots,N$, 
\begin{equation}\label{eq:angular invariance}
        p(\boldsymbol{\phi}|Y,D=d)=p^t(\boldsymbol{\phi}|Y)
\end{equation}
\end{assumption}
%Notice that the polar reparametrization $g(\cdot)$ is bijective and $p(r,\boldsymbol{\phi}|Y,D)=p(\boldsymbol{\phi}|Y,D)p(r|\boldsymbol{\phi},Y,D)$, then it is straightforward to arrive at the following corollary.
%\begin{corollary}
%When the assumption~\ref{assump:angularInvariance} is satisfied, then condional on $Y$, dataset shifts in $\mathcal{Z}$ if and only if norm shifts in $\mathcal{Z}$,
%\begin{equation}\label{eq:NormShifts}
%    p(\textbf{z}|Y,D)\neq p^t(\textbf{z}|Y,D) \leftrightarrow p(r|\boldsymbol{\phi},Y,D) \neq p^t(r|\boldsymbol{\phi},Y).
%\end{equation}
%\end{corollary}

Notice that the polar reparametrization $g(\cdot)$ is bijective and $p(r,\boldsymbol{\phi}|Y,D)=p(\boldsymbol{\phi}|Y,D)p(r|\boldsymbol{\phi},Y,D)$, therefore the difference between the target conditional p.d.f. (c.p.d.f.) $p^t(\textbf{z}|Y)$ and the $d$-th source c.p.d.f. $p(\textbf{z}|Y,d)$ is captured by the difference between the norm c.p.d.f.s $p^t(r|\boldsymbol{\phi},Y)$ and $p(r|\boldsymbol{\phi},d,Y)$.

%With the angular invariance, the next theorem formalize the intuition that the deference between the target conditional p.d.f. (c.p.d.f.) $p^t(\textbf{z}|Y)$ and the $d$-th source c.p.d.f. $p(\textbf{z}|Y,d)$ is captured by difference between the norm c.p.d.f.s $p^t(r|\boldsymbol{\phi},Y)$ and $p(r|\boldsymbol{\phi},d,Y)$.

\begin{theorem}\label{theorem:Reduce}
Suppose $support(p^t(\textbf{z}))\subset support(p(\textbf{z}|D))$. If the angular invariance assumption~\ref{assump:angularInvariance} holds, then for $d=1,\ldots,N$, $p^t(\textbf{z}|Y)/p(\textbf{z}|D=d,Y)$ exists and satisfies
\begin{equation}\label{eq:ratioweight}
 \frac{p^t(\textbf{z}|Y)}{p(\textbf{z}|d,Y)}=\frac{ p^t(r|\boldsymbol{\phi},Y)}{p(r|\boldsymbol{\phi},d,Y)}\triangleq w(r|\boldsymbol{\phi},d,y).
\end{equation}
\end{theorem} 

The theorem~\ref{theorem:Reduce} says that under the angular invariance assumption, we may reduce the degrees of freedom of comparing target and source c.p.d.f.s from $n$ to $1$. However, the aporia of DG is that no target instances could be observed during training. Thus an extra assumption is essential to overcome the zero-sample dilemma. Following the maximum entropy principle~\cite{jaynes1957information}, we adopt the following distributional assumptions on the conditional target and source norms.

\begin{assumption}[maximum entropy norm distribution]\label{assump:maximumEntropy} Conditioned on $Y=y$ and $\boldsymbol{\phi}$, (I) The target norm in space $\mathcal{Z}$ follows a continuous uniform distribution\footnote{The uniform distribution is the maximum (differential) entropy distribution for a continuous random variable with a fixed range.} $Uni[\alpha_{y,\boldsymbol{\phi}},\beta_{y,\boldsymbol{\phi}}]$ with $\delta_{y,\boldsymbol{\phi}}=\beta_{y,\boldsymbol{\phi}}-\alpha_{y,\boldsymbol{\phi}}>0$, i.e., $p^t(r|y,\boldsymbol{\phi};\alpha_{y,\boldsymbol{\phi}},\beta_{y,\boldsymbol{\phi}})=1/\delta_{y,\boldsymbol{\phi}}$. (II) The $d$-th source domain norm in space $\mathcal{Z}$ follows an exponential distribution\footnote{The exponential distribution is the maximum (differential) entropy distribution with positive support and a fixed expectation.} $Exp[1/\mu_{d,y,\boldsymbol{\phi}}],\mu_{d,y,\boldsymbol{\phi}}>0$, i.e., $p(r|d,y;\mu_{d,y,\boldsymbol{\phi}})=1/\mu_{d,y,\boldsymbol{\phi}} exp(r/\mu_{d,y,\boldsymbol{\phi}})$.% for $d=1,\ldots,N,y=1,\ldots,C$.
\end{assumption}

With the angular invariance and the maximum entropy assumption, we can compare $p^t(\textbf{z}|y)$ and $p(\textbf{z}|d,y)$ analytically.
\begin{corollary}\label{cor:RatioanalyticForm}
When assumption~\ref{assump:angularInvariance} and assumption~\ref{assump:maximumEntropy} hold,
\begin{equation}\label{eq:RatioanalyticForm}
    w(r|\boldsymbol{\phi},d,y)%= \frac{p^t(\textbf{z}|y)}{p(\textbf{z}|d,y)}
    =\frac{\mu_{d,y} exp(\frac{r}{\mu_{d,y,\boldsymbol{\phi}}})}{\delta_{y,\boldsymbol{\phi}}} \approx \frac{\mu_{d,y,\boldsymbol{\phi}}+r}{\delta_{y,\boldsymbol{\phi}}}.
\end{equation}
\end{corollary}

%Conditioned on the output class random variable $Y$, we have conclude the difference between the target and source latent representations $\textbf{Z}$ can be characterized by the c.p.d.f.s between the corresponding norms as in eq.~\eqref{eq:ratioweight} (and eq.~\eqref{eq:RatioanalyticForm}).
Recalling that DG aim to learn classifiers, next we consider the behavior when $Y$ varies, i.e., $p^t(y|\textbf{z})$ and $p(y|\textbf{z},D)$.

%\noindent \textbf{Angular Invariance Domain Generalization Network}\\
\subsection{The AIDGN Method}
Before the formal introduction of the proposed AIDGN method, We discuss the motivation of adopting the von-Mises Fisher (vMF) mixture model. Specifically, we inspect $p(\textbf{z}|Y)$ and $p(\boldsymbol{\phi}|Y)$, where $\boldsymbol{\phi}=(\phi_1,\ldots,\phi_{n-1})$ is the angular coordinates after a polar reparameterization of $\textbf{z}$. By the law of total probability, the source c.p.d.f. $p^s(\textbf{z}|Y)$ decomposes as
\begin{equation}\label{eq:totalSum}
    \begin{aligned}
    p^s(\textbf{z}|Y)&=\sum_{d=1}^N p(\textbf{z}|d,Y)p(d|Y)\propto \sum_{d=1}^N p(r,\boldsymbol{\phi}|d,Y)p(d|Y)
    \end{aligned}
\end{equation}
When the angular invariance and norm shift assumption~\ref{assump:angularInvariance} holds, the factors $p(\textbf{z}|d,Y)$ and $p(d|Y)$ might varies w.r.t. the domain index $d$. Therefore modeling $p^s(\textbf{z}|Y)$ urges the modeling of $p(\textbf{z}|d,Y)$ w.r.t. $d=1,\ldots,N$. In sharp contrast, the angular invariance guarantees the modeling of the source c.p.d.f. $p^s(\boldsymbol{\phi}|Y)$ is as easy as any $p(\boldsymbol{\phi}|Y,d)$ for $d=1,\ldots,N$. By eq.~\eqref{eq:angular invariance}, $p^s(\boldsymbol{\phi}|Y)=\sum_{d=1}^N p(\boldsymbol{\phi}|Y,d)p(d|Y)=p(\boldsymbol{\phi}|Y,d)\sum_{d=1}^N p(d|Y)=p(\boldsymbol{\phi}|Y,d)$.
%\begin{equation}\label{eq:AngularEasiness}
%\begin{aligned}
%    &p^s(\boldsymbol{\phi}|Y)=\sum_{d=1}^N p(\boldsymbol{\phi}|Y,d)p(d|Y)\\
%    &=p(\boldsymbol{\phi}|Y,d)\sum_{d=1}^N p(d|Y)=p(\boldsymbol{\phi}|Y,d).
%\end{aligned}
%\end{equation}
%According to eq.\eqref{eq:AngularEasiness}, the source joint p.d.f. $p^s(\textbf{z},y)$ boils down to inspecting the source c.d.p.f. $p^s(\boldsymbol{\phi}|y)$ and the source marginal p.d.f. $p^s(y)$. To this end, a natural choice is performing the $L_2$ normalization $\mathcal{G}(\textbf{z})$ of the latent representation $\textbf{z}$, 
Therefore, the much simpler assumption choice is a model related to $p^s(\boldsymbol{\phi})$.
Notice that the angular coordinates of the latent representation $\textbf{z}$ are invariant to the $L_2$ normalization $\mathcal{G}(\textbf{z})$, i.e., $\mathcal{G}\circ g: (r,\boldsymbol{\phi})\mapsto (1,\boldsymbol{\phi})$, where $g$ is the polar reparameterization and $\mathcal{G}(\textbf{z})$ is
\begin{equation}\label{eq:l2normalization}
    \mathcal{G}(\textbf{z})=\textbf{z}/\sqrt{z_1^2+z_2^2+\ldots+z_n^2}.
\end{equation}
The formulation of the proposed AIDGN begins with the vMF mixture assumption on the $L_2$ normalized $\mathcal{G}(\textbf{Z})$.

\begin{assumption}[von-Mises Fisher mixture]\label{assump:vMFMixture}
Suppose that the assumption~\ref{assump:angularInvariance} is satisfied, let $\textbf{Z}^*\triangleq \mathcal{G}(\textbf{Z})$ be the $L_2$ normalization of the latent representation $\textbf{Z}=\pi(\textbf{X})$. In the $C$-way DG classification setting, $\textbf{Z}^*$ is assumed to follow a von-Mises Fisher mixture distribution,
\begin{equation}\label{vMFmixture}
    p(\textbf{z}^*)=\sum_{y=1}^C p(Y=y)p(\textbf{z}^*|y)=\sum_{y=1}^C p(y)\mathcal{V}(\textbf{z}^*;\textbf{w}_y,\kappa),
\end{equation}
such that the posterior p.d.f. $p(y|\textbf{z},D)$ is invariant to the $L_2$ normalization, i.e.,
\begin{equation}%\remark:this equation implies assuming p(r|d,y,\phi)=p(r|d,\phi), \phi is encoding all categorical information of a source sample
    p(y|\textbf{z},D)=P(y|\textbf{z}^*,D).
\end{equation}
The $y$-th component of the mixture $p(\textbf{z}^*|y)=\mathcal{V}(\textbf{z}^*;\textbf{w}_y,\kappa)$ is the p.d.f. of a vMF distribution,
\begin{equation}\label{eq:vMFdistribution}
\mathcal{V}(\textbf{z}^*;\textbf{w}_y,\kappa)=\frac{\kappa^{n/2-1}}{(2\pi)^{n/2}I_{n/2-1}(\kappa)}exp(\kappa \textbf{w}_y^{\top}\textbf{z}^*),
\end{equation}
where $I_n$ denotes the first kind Bessel function at order $n$.
\end{assumption}

Within the vMF mixture model, the angular invariance induces a relationship between the target posterior $p^t(y|\textbf{z})$ and the source mixture components $p(\textbf{z}^*|y)$. % connected by the relative difference between $p^t(\textbf{z}|y)$ and $p(\textbf{z}|d,y,d)$.
\begin{theorem}\label{theorem:posterior}
When the assumptions~\ref{assump:angularInvariance} and~\ref{assump:vMFMixture} is satisfied, then 
\begin{equation}\label{eq:posterior}
\begin{aligned}
        p^t(y|\textbf{z})&=\frac{p(\textbf{z}^*|Y=y)w(r|\boldsymbol{\phi},d,y)P(Y=y)}{\sum_{c=1}^C p(\textbf{z}^*|Y=c)w(r|\boldsymbol{\phi},d,c)P(Y=c) }\\
        &=\frac{exp(\kappa \textbf{w}_y^{\top}\textbf{z}^*)w(r|\boldsymbol{\phi},d,y)P(Y=y)}{\sum_{c=1}^C exp(\kappa \textbf{w}_c^{\top}\textbf{z}^*)w(r|\boldsymbol{\phi},d,c)P(Y=c) }.
\end{aligned}
\end{equation}
\end{theorem}

The eq.~\eqref{eq:posterior} in theorem \ref{theorem:posterior} promises an optimization objective when there are enough observations for each source domain. However, the sample size is often  prohibitive and even if the sample complexity could be satisfied by the sample size, inputting too many source instances in mini-batches is not practical for a DNN. On the other hand, the empirical estimation of $w(r|\boldsymbol{\phi},d,c)$ likely equals to $0$ when the class index $c$ is not correct for a $d$-th domain instance $\textbf{z}$ with polar coordinates $(\boldsymbol{\phi},r)$, possibly because there is no such an instance in the training dataset at all.

The above practical concerns motivate us to modify eq.~\eqref{eq:posterior}. For ease of illustration, we rewrite the vMF exponent factors $\textbf{w}_y^{\top}\textbf{z}^*\triangleq cos(\theta_y), y=1,\ldots,C$. For a sample instance $(\textbf{z},y)$, the proposed AIDGN method reinterprets the influence of $w(r|φ,d,y)$ on $cos(\theta_y)$ as a modification on $\theta_y$ such that  $exp(\kappa cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))\approx exp(\kappa cos(\theta_y))w(r|\boldsymbol{\phi},d,y)$. And suppose that for the wrong classes $c\neq y$, $w(r|\boldsymbol{\phi},d,y)$ is upper bounded by $m>0$. Then optimizing $p^(y|\textbf{z})$ to be close to $1$ reduces to enforcing 
\begin{equation}
    cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y))p(y)\geq cos(\theta_c+\gamma m)p(c), % we take \gamma m =0 in our experiments
\end{equation}
where $c\neq y$ is indexing any wrong class of $(\textbf{z},y)$. To derive the optimization objective of AIDGN, we adopts the maximum entropy principle again on the label distribution.

\begin{theorem}\label{theorem:Loss}
Let $\Delta$ be a $C-1$ simplex and let $\textbf{P}=(P_1,\ldots,P_C) \in \Delta$ denote a distribution of classes, then
\begin{equation}\label{eq:labelMEP}
\begin{aligned}
    \textbf{P}^*&=(\frac{e^{\kappa(cos(\theta_1+\gamma m)-cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))}}{\sum_{c=1}^C e^{\kappa(cos(\theta_1+\gamma m)-cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))}}\\
    &\ldots,\frac{e^{\kappa(cos(\theta_C+\gamma m)-cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))}}{\sum_{c=1}^C e^{\kappa(cos(\theta_1+\gamma m)-cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))}})\\
    =&\arg \max_{\textbf{P}\in \Delta} \kappa [ \sum_{c\neq y}^C P_c( cos(\theta_c+\gamma m)-cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))\\
    &+P_y(cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)
     -cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y)))]\\
     &+\sum_{c=1}^C P_c(-log P_c).
\end{aligned}
\end{equation}
At $\textbf{P}=\textbf{P}^*$, the maximum of the right hand side (r.h.s.) is
\begin{equation}\label{eq:AIDGNloss}
\begin{aligned}
    &\ell_{AIDGN}(\textbf{z},y)\\
    &=-log \frac{e^{\kappa cos(\theta_y+w(r|\boldsymbol{\phi},d,y))}}{e^{\kappa cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y))}+\sum_{c\neq y}e^{\kappa cos(\theta_y+\gamma m)}}.
\end{aligned}
\end{equation}
\end{theorem}

In theorem~\ref{theorem:Loss}  eq.~\eqref{eq:AIDGNloss}, we derived the loss $\ell_{AIDGN}(\textbf{z},y)$. We next inspect the gradient behavior of the loss. We take the gradients of $\ell_{AIDGN}(\textbf{z},y)$ w.r.t. the correct center $\textbf{w}_y$ and w.r.t. an incorrect center $\textbf{w}_c$. At the $k$-th time step of training, denote by $\textbf{p}_k$ the prediction vector of the model 
\begin{equation}\label{eq:gradients}
\begin{cases}
    \partial \ell_{AIDGN}(\textbf{z},y)/\partial \textbf{w}_y \propto \kappa \left(1-p_k(y) \right) \textbf{z},\\
    \partial \ell_{AIDGN}(\textbf{z},y)/\partial \textbf{w}_c \propto \kappa p_k(c)\textbf{z}.
\end{cases}
\end{equation}

When performing the gradient descent training, the eq.\eqref{eq:gradients} reveals not only the ideal behavior of decreasing gap between correct prediction probability and 1, but also a non-ideal behavior in our DG formulation, i.e., shrinking the latent representation $\textbf{z}$. Specifically, when we assume the angular invariance, the norm of $\textbf{z}$ carries useful information for comparing $p^t(\textbf{z}|Y)$ and $p(\textbf{z}|D,Y)$ as discussed in theorem~\ref{theorem:Reduce}, and the shrinking of $\textbf{z}$ causes information loss in the norm coordinate.

To combat against the shrinking tendency brought by the $\ell_{AIDGN}(\textbf{z},y)$ loss, we introduce an information regularizer to penalize the loss of information. Concretely, we introduce an ideal norm distribution (which can be regard as the norm distribution of a perfect source domain) that follows an exponential distribution $Exp(1/\mu^*)$. The information loss regularizer $KL(\cdot \| \cdot)$ is the Kullback-Leibler (K-L) divergence \cite{Kullback1951On} that calculates the relative entropy~\cite{jaynes1957information} between $Exp(1/\mu^*)$ and $Exp(1/\mu)$.
\begin{equation}
  KL(1/\mu^* \|1/\mu)=log(\mu/\mu^*)+\mu^*/\mu-1
\end{equation}

Finally, the final optimization objective of the proposed AIDGN is 
\begin{equation}\label{eq:finalOO}
\begin{aligned}
        &L_{AIDGN}= \sum_{d=1}^N  \sum_{i=1}^{n_d} \eta KL(1/\mu^* \|1/\mu_{d,y,\boldsymbol{\phi}})\\
        &-log \frac{e^{\kappa cos(\theta_y+w(r|\boldsymbol{\phi},d,y))}}{e^{\kappa cos(\theta_y+\gamma w(r|\boldsymbol{\phi},d,y))}+\sum_{c\neq y}e^{\kappa cos(\theta_y+\gamma m)}},
\end{aligned}
\end{equation}
where $\eta>0$ is a hyperparameter controlling the trade-off between information memorizing and forgetting.

\begin{remark}
The proposed AIDGN optimization objective eq.~\eqref{eq:finalOO} theoretically justifies and generalizes the recent proposed MAG loss for face recognition~\cite{meng2021magface}. When there is only one source domain, it can be easily verified that with a first order Maclaurin's expansion approximation w.r.t. the log term in the regularizer $KL(1/\mu^* \|1/\mu)$, the proposed AIDGN loss eq.~\eqref{eq:finalOO} degenerated to the MAG loss.
\end{remark}




%For $K$-way classification problem, we assume our model consists of a feature extractor $f_{\theta}(\cdot)$ and $K$ class centers $\lbrace c_k \in \mathbb{R}^{z}, k=1,...,K\rbrace$. For each input sample $x_i^d$, its $z$-dimension embedding $f_i^d=f_{\theta}(x_i^d)$ is computed by the feature extractor and is used to compute cosine similarity with each class center $c_k$, then the category with the largest cosine similarity between its class center and the sample will be output as the label prediction.

%Following~\cite{meng2021magface}, we use the magnitude of each feature, i.e, $a_i^d=\lVert f_i^d \rVert_{2}$, to denote the quality of the sample. Moreover, we additionally introduce two indicators to measure the quality of each source domain. We denote the mean and standard deviation of sample magnitudes in domain $d$ by $e_d$ and $s_d$, respectively. Intuitively, a high-quality domain should have a larger mean and smaller deviation, and thus is more important in training a model with better generalization ability.







==> Sect/related_work.tex <==
\section{Related Work}

Domain generalization (DG) aims at generalizing the model trained on multiple source domains on perform well on related but unseen target domains. Compared with domain adaptation (DA), DG deals with a more practical yet challenging setting where the target domain data is unavailable during training. A common pervasive theme in DG literature is domain-invariant representation learning, which is based on the idea of aligning features among different source domains, with the hope that the learned  invariance can be generalized to target domains. For instance, ~\cite{li2018mmd} achieved distribution alignment in the latent space of an autoencoder by using adversarial learning and the maximum mean discrepancy criteria. ~\cite{li2018cdann} instead resorted to matching conditional feature distributions across domains, enabling alignment of multimodal distributions for all class labels. ~\cite{liu2021ijcai21} exploited both the conditional and label shifts in various DG tasks, and proposed a Bayesian variational inference framework with the posterior alignment to reduce both the shifts simultaneously.

Meta-learning was introduced into the DG community by~\cite{li2018mldg} and has drawn increasing attention. The main idea is to divide the source domains into meta-train-domains and meta-test-domain to simulate domain shift, and regulate the model trained on meta-train-domains to perform well on meta-test-domain. Data augmentation has also been exploited for DG, which augments the source data to increase the diversity of training data distribution. For instance, ~\cite{wang2020mixup} employed mixup~\cite{zhang2018mixup_origin} technique across multiple domains and trained model on the augmented heterogeneous mixup distribution, which implicitly enhanced invariance to domain shifts. Despite great progress has been made in DG, ~\cite{gulrajani2020domainbed} found that with careful implementation, empirical risk minimization method outperforms various state-of-the-art methods in DG.

Different from the above methods which focus on training phase, test-time adaptation is a class of methods focusing on test phase, i.e., adjusting the model using online unlabeled data and correcting its prediction by itself during test time. ~\cite{wang2020Tent} proposed fully test-time adaptation, which modulates the BN parameters by minimizing the prediction entropy using stochastic gradient descent. ~\cite{iwasawa2021T3A} proposed a test-time classifier adjustment module for DG, which continually updates pseudo-prototypes for each class using online unlabeled data augmented by the base classifier trained on the source domains. We empirically find that multiple test-time adaptation methods based on entropy minimization cannot further improve the performance of the model trained under our proposed framework. 




